Masked Autoencoder Pretraining on Strong-Lensing Images for Joint Dark-Matter Model Classification and Super-Resolution

Strong gravitational lensing can reveal the influence of dark-matter substructure in galaxies, but analyzing these effects from noisy, low-resolution images poses a significant challenge. In this work, we propose a masked autoencoder (MAE) pretraining strategy on simulated strong-lensing images from the DeepLense ML4SCI benchmark to learn generalizable representations for two downstream tasks: (i) classifying the underlying dark matter model (cold dark matter, axion-like, or no substructure) and (ii) enhancing low-resolution lensed images via super-resolution. We pretrain a Vision Transformer encoder using a masked image modeling objective, then fine-tune the encoder separately for each task. Our results show that MAE pretraining, when combined with appropriate mask ratio tuning, yields a shared encoder that matches or exceeds a ViT trained from scratch. Specifically, at a 90% mask ratio, the fine-tuned classifier achieves macro AUC of 0.968 and accuracy of 88.65%, compared to the scratch baseline (AUC 0.957, accuracy 82.46%). For super-resolution (16x16 to 64x64), the MAE-pretrained model reconstructs images with PSNR ~33 dB and SSIM 0.961, modestly improving over scratch training. We ablate the MAE mask ratio, revealing a consistent trade-off: higher mask ratios improve classification but slightly degrade reconstruction fidelity. Our findings demonstrate that MAE pretraining on physics-rich simulations provides a flexible, reusable encoder for multiple strong-lensing analysis tasks.

==> outputs_lens/classifier/data/76 <==
¢6L?5–>\åq?™g?°È[?g}s?hQg?ŸTü>â'^?)i?z»Y?'6??[Õ?´êS?ª"X?K0?0J?ՌG?~J_?· t?Íáh?ݞv?GwN?Y4g?ʳ[?BbW?"ò\?ÁØg?ÀÈ=? 'E?B g?:³§>Ävs?Èëb?|xX?êf?óÄk?jg?i»C?Ÿ-(?¢`?­9q?¿Ê_?1U?ãÔ?¹ö*?×ÞM?þ"H?'G?$/\?tÛ_?ÂwK?¤^?÷A`?}?~8…>R¾V?ˆäQ?©—æ>þl]?@]?±W]?8:W?­n·>ðä?4[q?±Ðs?átI?w%Z?9v??+Ýi?–MJ?§Û\?È3i>­k?Þ»%?')?ž\¨>íV?jA?Þ¤^?&K?ä3?¡U?j.Î>è¤0?Š,?…µX?Ü"U?_Ž?¿º?ŸCª>À³Ÿ>(ÓG?Чl?‰çS?é,Î>`?D?ã¬u?`?a+Ï>®Lj?3*P?	Ç+?…¥j?"c?Ţ>ä†P?ŒîW?»éS?öH?ò|Z?Šo>èê>ƒf?¾³u?ÈèQ?ÐúR?ÓË3?þ_?ÕV>?€I?'ô!?Ñ ?v*H?ûGR?ºÑ¿>¸Å^?;(B?¬'J?mÛ2?¿f?‹7?mF?Qd?‹*x>iÊS?3ÌP?¿Åc?»g?Ãé?èp?	,?ð3?<µ?`V?õ`?+©^?
r?WqL?©?+M?÷ýp?(ša?»">¤ÇX?)ä_?HùG?éA?WX?Z_?Ó/?¯/a?–KL?ñ>­>Ér:?-¥X?k?HuI?rºq?çwR?U´\?g)?þ¥?'Z?€®`?d+b?¦O?íúd?²l?çøŽ>íñm?ŸT?я_?ð¸n?8®a?àË`?nZ?¿¥h?´N?'ê(?cfp?

==> outputs_lens/sr_model/data/29 <==
³he9.J8
Bä9âŠ9Þ [94΅7¿Íä9]‡T9·¦9«Ò8å)Ù60\À¸

]¹i_
9eο8üÀ¸9®ZE¹ÆÃ[¸«¥8B5¹Ñ𹩟¹œqd8½M¹Øÿ8ºÖ9Û5 ®¸wט8%}:Вkµt{9ב9ûîy9tàô¹‹û.¹GïY¹E`76?÷¹oq`¹´M«¹Žt—¹5:ùø¹2›Í¸ôon¹g﮸0T¹PrŽ¸~šÖ9
º†™"9»_^9Õ˸uqT7Þ$v9ᘝ¸«3*9z@¹Þ)»¹ãÞ;¹<õÜ9É]9b=¯¸ž3¸¢‰9¦‰¹Ŏ8Àk7¸EU¥8ß¹{¹{0í7¿q9KîǸÝÊ&:©&«¸ô •8$ØH¹X²Z·}šp8ä.ê9¶Oƒ¸ x†9ö5¹€,º&¸™b9Ž{‡¹+@o¹›–M¹"î7±ñ)¹6ß¹»¨ì9~Øk¹q¼'¹óW¹\
°¸æ5±8hm8£Áø·ˆr…¹`uœ¹ª"À9Û|M¹W«:¹šï¹v…ë8¹k¹lÒ¹i¡9Ϝµ8¾¦¹h»8Õb'9*j%79²Ñ7ˆ64¹ö¶ú¸¥F¹Rò¹1áç¹äP9gŸË¹¢²8y™8—ýÀ9¦ò之+i9ÖÆW9l•=9mg«9k¬¶9ê/^9
Ëò·÷`
º&¨Ó¹í"9Õ´ 8ÆJQ¹Ґ90†Œ9.*Z6±)¶¹?\d¸§¢¸˜pz7|¹8\ç‰9s)¹ÏÃ	8Ò\´¸‡j-8¼d¸ˆ.Ù6»¯7dĸùn¸G¥&¹¨J¹<‡Å¹éûg9Œ;ºknÓ8Éc¹@&9âi+99帹¼½B¹Nu"·J.M¹$J÷¸Ì°9›ë	¹È3 :F¿µ¸±&‰¶ݬ9X­e8ôÞü8ªPÌ9Ö¡9CK«9…(-º†—$¹
A¹ö*Ô8ç¬N:ºyÿ¹ûé¬8õï¹+g9

==> outputs_lens/sr_model/data/34 <==
èâb?ëÜb?º'c?Öb?R[c?xîb?֛d?Ú	c?,1c?ñRb?¶äb?<e?74c?Õ¿b?U½b?hÓb?ÔÚb?§Ôb?äÌb?\ðb?.îb?¬Tc?Kìb?
8d?‡ c?Rc?Mµb?ù]c?y'c?¿b?!$c?†tc?"jf?½îb?åc?‡­c?Ô|c?eìb?¡éb?"éb?,&c?†6c?lc?+c?¢c?ŠÙb?@Èb?Ìb?åc?Ëýb?Øb?DKc?yùb?†²b?Óc?Úc?,c?(øb?'c?µc?Ùb?Zc?µùb?aéb?óôb?ñºb?¶6c?À:c?Þ
c?–Ãb?Ë5c?A%c?.îb?=4c?
c?ïxc?c?–b?´Æb?Ò®c?wÈc?âc?äc?_ˆc?zZd?~c?V°c?7dd?–c?‹òb?L§c?öíb?Ûc?…¦c?ß0c?'uc?äc?Ôc?+je?ó*c?/Ùb?Üc?wËb?)d?Àíb?EÚb?•c?Ø0c?]>c?c?ùb?Jºb?L¤d?Àb?Lêb?Юc?";c?LÑd?Ôc?%7c?Êc?Hc?¯úb?átc?p-c?Âb?òíb?À¡b?©Sd?PÞb?Îb?ºc?sÙb?‡$c?Úc?O¿b?ޚc?ec?Hc?.c?2bc?gØc?æ\d?=ñc?Bc?8çb?^Èc?†bc?Û`d?(¹b?-éb?ìc?u©b?÷c?ß/c?½
d?ñc?™c?ôb?Šc?Ø
c?…Hc?­êb?zïb?¹êb?Á3c?š²b?
c?J´b?âc?©Pc?f?¹c?Èb?á2c?Áúb?Ëb?¼åb?&b?Ñb?(òb??d?êb?u®b?´c?‹Sc?Fjc?'@d?nÚb?Uêb?m¾c?¤šc?

==> outputs_lens/sr_model/data/47 <==

ÊÃ7HǏ¸Ô~!¹#0¸9–j7þÿ28'¤£9'!æ·k+É7oç7W\¸«'‹¹Ž'¶»ß{·Ã«Ž7r·x%n9ð·â·üR¸MZ	8<ò¢7ÃìÄ6Å`͸Êà·ÈÈÀ7iª«7° ·F
¯8=Ä©¸í¸iÚT8ôÔ8SÏ7Œ˜·Vh~¸uáL¸‹$n8³y´7I7I¸íCb9¨¢7ÑF·Çf7'áB9žê¸¸U[ý±·×÷†·epä·cºK7"¯7÷—å·F=¸Kuïµeû?8_ ¹,·à=¾8ü°¥¹9ä7˜?7*>·ZJ•·9â· j9Oµ8Éÿ–¸3Bö¶"
N5 h—8Óû'¸eٕ8-m•8®j9Lµ¸õB$9Uç¢7ŽŸ8´ïâ¸F:p7¡"›¸Ÿ'€µþ7¿	¸6·×8<IÔ¶Ä>¸op6–Æg4°TR¸ûQ"8åXŠ¸ž·5$H¸ß"—8CtÝ7µÊ6¸
{8JE	º÷^ý6oµ7zN·³êà7-ɹ·7—¹†@"¸³IÄ76:¹.çü7¶ðP¸8´=¹ÊĸNÛi¸B‹š7¼që8!»S9¢}·ûÐ8°˜ª8þ᣶#só·sH8š¹xk¹Ë®p7Õ3Ÿ7*Í̶ª¦½8kï!¸¨Ùï¸SÔ»·"µß7Ò®"8îþà7ª~˜·ì<Ð7?œc¶Ö&8u(¸R‹[8–϶… ¸›â¶Æ]"¶îÕõ·§Š¨¸
·T8ŽHž¹wøá7c§â7§b}¸Ð'j8¯47=í†8¿þA8‹þ%¸c00·Ê›O7ZÅ*·"O¤5»›Ì7šÊÒ·A±'·2¹íå'7cf=·ªþ6×&Ÿ8G]%8¢ç 8òÈ)¸J6Æÿ›8"ÊÈ·Ö·í79ב7z¶·ÏЎµžâ{7©èp·38Þm{·}‰Ê·•'–¸qüv·2È 6ôק8l÷E·ÆX/·_¢7Æ.ƒ¹

==> outputs_lens/sr_model/data/59 <==
ßÿ7äQ39<"9Hœ9êq·Ol™8Ïu*8Öf¹«NX7ͤw7	.7'©·½Ò¶09Ž·9:.8ƒ·ƒþ‹7m{‹7€bi¶Øˆˆ71"Ã6?5"8º…·Ô̏7|Õ·}ËÅ62š¶}ƒ8øw6˾¶÷B¼·FPi7W–
8Ê®ƒ¸þ¶¦·>ƒ¸¶óŠ64–J6žô·ÜÜ1¶£.¯7RÁµ#·²¶¶.¶Z^a¸•¸(W"7!4Ý6­=º¶—ëù8E¶7ò{B8r•%64z·î›8%q›6Eiþ·Ù¨&8¼à"¸î»~6‹¦85›8"±3·%c7ÿG·¥F±6ZÍ=¸»™77c·ì^7`·V¸ëL£72ñ¸*PP8¡Û«¸ê5œ7t$Æ50¼y7°ÂA7ƒp(·:Ä6øÔ8Ʀ¸^-™7þNÿ6‹Æ¬·+Î6í¨Í7½y7BøÎ5 ¬7A¤4·²c¸7A쟸áY¿·È½'¶{"·*'Ð7×2Y·ër˜·&e¸%¼†¸ëù6à‡b¸akÉ·µ¦Q8'ˆ\·Àe`8­ÖM93¸¸¯¶£¯ 8Ñ£Ú³áÅS7ø7Ã9¾<¯¶6¥:h$í´yò‡¶|½Y7Z*Ù7eÉl¸…†Ø7mi·þŽ7©…·žX츈ÝÅ6®ý™6Ï~¦µæœ¿8"'|¸kQ&¶~f–·=¸¤e"·Ž~¯·_·¸S¾7"d¨·^"½85‡Å¸ï´µöV·^Ô"·hpÎ7æ%
·¹ŽW¸NH.¹r½Œ7­¿þ8–LK·ºh–6˜/"8¾…†8çô–¸ÃPe·Y£;· ý.9óÉh·Bïp¹;1Ž·ùþ¸P1*7 ai8»¸f¸ÛG©8£_¸º~q827¹6P
]6§g`¹}¸uÖ­¶o)¤µ S¦¶×#7á—µT‹2¹ô¾G·wݙ·u¥L7îg¸·%Վ8øBθŽj77ñ'¸ë¥'8[Ž7Rb¯¹

==> outputs_lens/sr_model/data/71 <==
ð?8vCœ5:ð:8ë«¡7ÃÆ+8¢a7;4ñ7èüê7›¾A8•[7Ïý7¦ÐµcyඪÉà¶
7»Ñ¥¹ã·^€·ªG17Âû!¸Š¼"6,59ˆì8àÎË8ÄLŸÇúÓ¶ã띶­ya·G÷k•·\ú6ñš7±á«9ζBV4¸8–9Ɂ8 dq¶}(¸–-5Q¹·EêÆ7ó)~7Œ¥Œ8bÚĶ!/R98?9»´7@º6."9w¸tÁ77uV
·«UÆ6ù)09éÚZ7Nvé·UÓ\7ˆ»E7®Þ8©ï¥¸
QZ6ó"ðµßзã«¶fžâ·€Ñà8µ8.š·£?¶{5¸rØ[8G™Å¶ô­ë¸ڞ¸õ|…¸;ÞL·¢æ
·±öh¶.£ˆ¶÷»8Å	¶7NC¸×Ɖ69zž7"Êx·¦Û·å6eº·ºòž¶1¸"ü8OÚ7Iå¸÷«½·ÁÅÙ¶-pR·Øþ8µ5œ¸åm'8~ZŽ7ñ¼·ft¸þ$¸5Fڑ¶í]¶ƒ¸B×µº¢ÿ8hž6Yéj6xÎk7<Ȝ·Î­V7cŽ¶<x7@à7ä½7ÖoÓ8'N‹7
¸·OÆi7ӗ!¸""·û/76*𸟾¹é¶97ç78'í´ÛwÌ7¿n6²þ·('µ>Z
·£1¹¸Ñ"¹7é´þ>É·/8Â8&fï6Ú£b8ûJ47ï­m9åþ	·lPý¶o7ë"o¶²t8dbš·¼¦‹¸­«¹JÅJ·Þï€8@Í8¹©¸3&ë¶uB·Ëí¸‡0⸂¼¸yöp¹þu(7™|Ž¸½A 6ÚN_¹Øô¶µ3>¹8›½¸áÈ79‡'+·Y-¿7Ó7=Ó·Tm!¸ÆÝ	71Ú¸æÁ€7Aäj¶s_(¸Üá3¶ž£µ­Y¢6›í^6²y	9å¸'¼]¸Ÿ¤07?±§7†P¸íw5´oÄ·

==> outputs_lens/sr_model/data/9 <==
Qg:át9oáÈ:‡P!:Ä#­8"¨ºZ±ˆ:µ}¢:ªA¸e*¹:­ŽÃ¹g˜9ýŒP9%_¸:bcº7QË·Ôßκ»‹sº0‰99ºbžÔºÖ²;ìW):l±/:0:KÍ¹"êÆ8~:³œiºxº51»<dï9©þ;:Çȹ}Q:šb,;ĵ:Æòn:ø|N¹6™N9÷Ì;º¤¬:
W½8i¨B9÷¹©®*:z,¢ºMó	¹`¿y:_±9A³:®4¨:™::,Tõ9XBÿ¹£(8+‰ºâëºÁB™:]þ
¹ËÜë¹ï§›9huº¹÷¹ì¨¡ºÒà7:Á©Þ9Ëc88,Âñº†›¹íh/ºú:°Yk¹¢kºÝßwº¾Øº«±ºî‡'ºHl€¸!ºXº=a—º9µ:iJ8°U*:I̹ºººôÎBÕ:'WÌ9-°Sº2…å:  ºKŒâ:ŸŒ:<QÈ9L­ºYr€¸S˜::%¹\ºº°u›9Â7Ê9!Ð:¿*2¹õú_ºf9?k»9jl9#¸m: YXº¯þº\[¡ºÕ!"ºxÇ8–"ºŽ:ŒÖ)¹ùmǺõÒÿ9ñæ9ÈZ¹ÑR¹$¹pºˆk0ºÆÍ09Í*ª:pk5:}Dl9OpÏ:Hÿ«¹KŒ»c¶¹•÷):-Ž¶xá¹Vʶ7(|¼ºÐùš9bVºe2‹:®½¹w©$;j8£9…hü:º'F:<Ùù¹Ãŀ¹Å\å9qm8ó©9:¨6pLJ9ô+9žº‡Ñ¸Uº‰6¡:QµºÀr¤:ŸwB¹x¢€º'F9ãä9ðםºC…·ºA:1ùs9~¯À¹õ>Ѻ'Ts:œ ˜·Ý\D;Sº·%ü·Öc›ºžvØ:Ðí;(%:}:aZ»~ñŽ:–û»Éè<9ÈA¹Ž{¥:N+:^:Ø]í¹!ªž¸¦øJºZ<.º
